In-situ calibration of the single-photoelectron charge response of the IceCube photomultiplier tubes

We describe an improved in-situ calibration of the single-photoelectron charge distributions for each of the in-ice Hamamatsu Photonics R7081-02[MOD] photomultiplier tubes in the IceCube Neutrino Observatory. The characterization of the individual PMT charge distributions is important for PMT calibration, data and Monte Carlo simulation agreement, and understanding the effect of hardware differences within the detector. We discuss the single photoelectron identification procedure and how we extract the single-photoelectron charge distribution using a deconvolution of the multiple-photoelectron charge distribution.

==> In-situ calibration of the single photoelectron charge response of the IceCube photomultipliers/authorlist.tex <==
\author[p]{M.~G.~Aartsen,}
\author[bc]{M.~Ackermann,}
\author[p]{J.~Adams,}
\author[l]{J.~A.~Aguilar,}
\author[t]{M.~Ahlers,}
\author[at]{M.~Ahrens,}
\author[z]{C.~Alispach,}
\author[ak]{K.~Andeen,}
\author[az]{T.~Anderson,}
\author[l]{I.~Ansseau,}
\author[x]{G.~Anton,}
\author[n]{C.~Arg{\"u}elles,}
\author[a]{J.~Auffenberg,}
\author[n]{S.~Axani,}
\author[a]{P.~Backes,}
\author[p]{H.~Bagherpour,}
\author[aq]{X.~Bai,}
\author[ac]{A.~Balagopal~V.,}
\author[z]{A.~Barbano,}
\author[ab]{S.~W.~Barwick,}
\author[bc]{B.~Bastian,}
\author[aj]{V.~Baum,}
\author[l]{S.~Baur,}
\author[h]{R.~Bay,}
\author[r,s]{J.~J.~Beatty,}
\author[bb]{K.-H.~Becker,}
\author[k]{J.~Becker~Tjus,}
\author[as]{S.~BenZvi,}
\author[q]{D.~Berley,}
\author[bc,bd]{E.~Bernardini,}
\author[ad,be]{D.~Z.~Besson,}
\author[h,i]{G.~Binder,}
\author[bb]{D.~Bindig,}
\author[q]{E.~Blaufuss,}
\author[bc]{S.~Blot,}
\author[at]{C.~Bohm,}
\author[u]{M.~B{\"o}rner,}
\author[aj]{S.~B{\"o}ser,}
\author[ba]{O.~Botner,}
\author[a]{J.~B{\"o}ttcher,}
\author[t]{E.~Bourbeau,}
\author[ai]{J.~Bourbeau,}
\author[bc]{F.~Bradascio,}
\author[ai]{J.~Braun,}
\author[z]{S.~Bron,}
\author[bc]{J.~Brostean-Kaiser,}
\author[ba]{A.~Burgman,}
\author[a]{J.~Buscher,}
\author[al]{R.~S.~Busse,}
\author[z]{T.~Carver,}
\author[f]{C.~Chen,}
\author[q]{E.~Cheung,}
\author[ai]{D.~Chirkin,}
\author[av]{S.~Choi,}
\author[ae]{K.~Clark,}
\author[al]{L.~Classen,}
\author[am]{A.~Coleman,}
\author[n]{G.~H.~Collin,}
\author[n]{J.~M.~Conrad,}
\author[m]{P.~Coppin,}
\author[m]{P.~Correa,}
\author[ay,az]{D.~F.~Cowen,}
\author[as]{R.~Cross,}
\author[f]{P.~Dave,}
\author[m]{C.~De~Clercq,}
\author[az]{J.~J.~DeLaunay,}
\author[am]{H.~Dembinski,}
\author[at]{K.~Deoskar,}
\author[aa]{S.~De~Ridder,}
\author[ai]{P.~Desiati,}
\author[m]{K.~D.~de~Vries,}
\author[m]{G.~de~Wasseige,}
\author[j]{M.~de~With,}
\author[v]{T.~DeYoung,}
\author[n]{A.~Diaz,}
\author[ai]{J.~C.~D{\'\i}az-V{\'e}lez,}
\author[av]{H.~Dujmovic,}
\author[az]{M.~Dunkman,}
\author[aq]{E.~Dvorak,}
\author[ai]{B.~Eberhardt,}
\author[aj]{T.~Ehrhardt,}
\author[az]{P.~Eller,}
\author[ac]{R.~Engel,}
\author[am]{P.~A.~Evenson,}
\author[ai]{S.~Fahey,}
\author[g]{A.~R.~Fazely,}
\author[q]{J.~Felde,}
\author[h]{K.~Filimonov,}
\author[at]{C.~Finley,}
\author[ay]{D.~Fox,}
\author[bc]{A.~Franckowiak,}
\author[q]{E.~Friedman,}
\author[aj]{A.~Fritz,}
\author[am]{T.~K.~Gaisser,}
\author[ah]{J.~Gallagher,}
\author[a]{E.~Ganster,}
\author[bc]{S.~Garrappa,}
\author[i]{L.~Gerhardt,}
\author[ai]{K.~Ghorbani,}
\author[y]{T.~Glauch,}
\author[x]{T.~Gl{\"u}senkamp,}
\author[i]{A.~Goldschmidt,}
\author[am]{J.~G.~Gonzalez,}
\author[v]{D.~Grant,}
\author[ai]{Z.~Griffith,}
\author[as]{S.~Griswold,}
\author[a]{M.~G{\"u}nder,}
\author[k]{M.~G{\"u}nd{\"u}z,}
\author[a]{C.~Haack,}
\author[ba]{A.~Hallgren,}
\author[a]{L.~Halve,}
\author[ai]{F.~Halzen,}
\author[ai]{K.~Hanson,}
\author[ac]{A.~Haungs,}
\author[j]{D.~Hebecker,}
\author[l]{D.~Heereman,}
\author[a]{P.~Heix,}
\author[bb]{K.~Helbing,}
\author[q]{R.~Hellauer,}
\author[y]{F.~Henningsen,}
\author[bb]{S.~Hickford,}
\author[w]{J.~Hignight,}
\author[b]{G.~C.~Hill,}
\author[q]{K.~D.~Hoffman,}
\author[bb]{R.~Hoffmann,}
\author[u]{T.~Hoinka,}
\author[ai]{B.~Hokanson-Fasig,}
\author[ai,be]{K.~Hoshina,}
\author[az]{F.~Huang,}
\author[y]{M.~Huber,}
\author[ac,bc]{T.~Huber,}
\author[at]{K.~Hultqvist,}
\author[u]{M.~H{\"u}nnefeld,}
\author[ai]{R.~Hussain,}
\author[av]{S.~In,}
\author[l]{N.~Iovine,}
\author[o]{A.~Ishihara,}
\author[e]{G.~S.~Japaridze,}
\author[av]{M.~Jeong,}
\author[ai]{K.~Jero,}
\author[d]{B.~J.~P.~Jones,}
\author[a]{F.~Jonske,}
\author[a]{R.~Joppe,}
\author[ac]{D.~Kang,}
\author[av]{W.~Kang,}
\author[al]{A.~Kappes,}
\author[aj]{D.~Kappesser,}
\author[bc]{T.~Karg,}
\author[y]{M.~Karl,}
\author[ai]{A.~Karle,}
\author[x]{U.~Katz,}
\author[ai]{M.~Kauer,}
\author[ai]{J.~L.~Kelley,}
\author[ai]{A.~Kheirandish,}
\author[av]{J.~Kim,}
\author[bc]{T.~Kintscher,}
\author[au]{J.~Kiryluk,}
\author[x]{T.~Kittler,}
\author[h,i]{S.~R.~Klein,}
\author[am]{R.~Koirala,}
\author[j]{H.~Kolanoski,}
\author[aj]{L.~K{\"o}pke,}
\author[v]{C.~Kopper,}
\author[ax]{S.~Kopper,}
\author[t]{D.~J.~Koskinen,}
\author[j,bc]{M.~Kowalski,}
\author[y]{K.~Krings,}
\author[aj]{G.~Kr{\"u}ckl,}
\author[w]{N.~Kulacz,}
\author[ap]{N.~Kurahashi,}
\author[b]{A.~Kyriacou,}
\author[aa]{M.~Labare,}
\author[az]{J.~L.~Lanfranchi,}
\author[q]{M.~J.~Larson,}
\author[bb]{F.~Lauber,}
\author[ai]{J.~P.~Lazar,}
\author[ai]{K.~Leonard,}
\author[ac]{A.~Leszczy{\'n}ska,}
\author[a]{M.~Leuermann,}
\author[ai]{Q.~R.~Liu,}
\author[aj]{E.~Lohfink,}
\author[al]{C.~J.~Lozano~Mariscal,}
\author[o]{L.~Lu,}
\author[z]{F.~Lucarelli,}
\author[m]{J.~L{\"u}nemann,}
\author[ai]{W.~Luszczak,}
\author[h,i]{Y.~Lyu,}
\author[bc]{W.~Y.~Ma,}
\author[ar]{J.~Madsen,}
\author[m]{G.~Maggi,}
\author[v]{K.~B.~M.~Mahn,}
\author[o]{Y.~Makino,}
\author[a]{P.~Mallik,}
\author[ai]{K.~Mallot,}
\author[ai]{S.~Mancina,}
\author[l]{I.~C.~Mari{\c{s}},}
\author[an]{R.~Maruyama,}
\author[o]{K.~Mase,}
\author[q]{R.~Maunu,}
\author[ag]{F.~McNally,}
\author[ai]{K.~Meagher,}
\author[t]{M.~Medici,}
\author[s]{A.~Medina,}
\author[u]{M.~Meier,}
\author[y]{S.~Meighen-Berger,}
\author[u]{T.~Menne,}
\author[ai]{G.~Merino,}
\author[l]{T.~Meures,}
\author[v]{J.~Micallef,}
\author[l]{D.~Mockler,}
\author[aj]{G.~Moment{\'e},}
\author[z]{T.~Montaruli,}
\author[w]{R.~W.~Moore,}
\author[ai]{R.~Morse,}
\author[n]{M.~Moulai,}
\author[a]{P.~Muth,}
\author[o]{R.~Nagai,}
\author[bb]{U.~Naumann,}
\author[v]{G.~Neer,}
\author[y]{H.~Niederhausen,}
\author[v]{M.~U.~Nisa,}
\author[v]{S.~C.~Nowicki,}
\author[i]{D.~R.~Nygren,}
\author[bb]{A.~Obertacke~Pollmann,}
\author[ac]{M.~Oehler,}
\author[q]{A.~Olivas,}
\author[l]{A.~O'Murchadha,}
\author[at]{E.~O'Sullivan,}
\author[h,i]{T.~Palczewski,}
\author[am]{H.~Pandya,}
\author[az]{D.~V.~Pankova,}
\author[ai]{N.~Park,}
\author[aj]{P.~Peiffer,}
\author[ba]{C.~P{\'e}rez~de~los~Heros,}
\author[a]{S.~Philippen,}
\author[u]{D.~Pieloth,}
\author[l]{E.~Pinat,}
\author[ai]{A.~Pizzuto,}
\author[ak]{M.~Plum,}
\author[aa]{A.~Porcelli,}
\author[h]{P.~B.~Price,}
\author[i]{G.~T.~Przybylski,}
\author[l]{C.~Raab,}
\author[p]{A.~Raissi,}
\author[t]{M.~Rameez,}
\author[bc]{L.~Rauch,}
\author[c]{K.~Rawlins,}
\author[y]{I.~C.~Rea,}
\author[a]{R.~Reimann,}
\author[ap]{B.~Relethford,}
\author[ac]{M.~Renschler,}
\author[l]{G.~Renzi,}
\author[y]{E.~Resconi,}
\author[u]{W.~Rhode,}
\author[ap]{M.~Richman,}
\author[i]{S.~Robertson,}
\author[a]{M.~Rongen,}
\author[av]{C.~Rott,}
\author[u]{T.~Ruhe,}
\author[aa]{D.~Ryckbosch,}
\author[v]{D.~Rysewyk,}
\author[ai]{I.~Safa,}
\author[v]{S.~E.~Sanchez~Herrera,}
\author[u]{A.~Sandrock,}
\author[aj]{J.~Sandroos,}
\author[ax]{M.~Santander,}
\author[ao]{S.~Sarkar,}
\author[w]{S.~Sarkar,}
\author[bc]{K.~Satalecka,}
\author[a]{M.~Schaufel,}
\author[ac]{H.~Schieler,}
\author[u]{P.~Schlunder,}
\author[q]{T.~Schmidt,}
\author[ai]{A.~Schneider,}
\author[x]{J.~Schneider,}
\author[ac,am]{F.~G.~Schr{\"o}der,}
\author[a]{L.~Schumacher,}
\author[ap]{S.~Sclafani,}
\author[am]{D.~Seckel,}
\author[ar]{S.~Seunarine,}
\author[a]{S.~Shefali,}
\author[ai]{M.~Silva,}
\author[ai]{R.~Snihur,}
\author[u]{J.~Soedingrekso,}
\author[am]{D.~Soldin,}
\author[q]{M.~Song,}
\author[ar]{G.~M.~Spiczak,}
\author[bc]{C.~Spiering,}
\author[bc]{J.~Stachurska,}
\author[s]{M.~Stamatikos,}
\author[am]{T.~Stanev,}
\author[bc]{R.~Stein,}
\author[ac]{P.~Steinm{\"u}ller,}
\author[a]{J.~Stettner,}
\author[aj]{A.~Steuer,}
\author[i]{T.~Stezelberger,}
\author[i]{R.~G.~Stokstad,}
\author[o]{A.~St{\"o}{\ss}l,}
\author[bc]{N.~L.~Strotjohann,}
\author[a]{T.~St{\"u}rwald,}
\author[t]{T.~Stuttard,}
\author[q]{G.~W.~Sullivan,}
\author[f]{I.~Taboada,}
\author[k]{F.~Tenholt,}
\author[g]{S.~Ter-Antonyan,}
\author[bc]{A.~Terliuk,}
\author[am]{S.~Tilav,}
\author[v]{K.~Tollefson,}
\author[k]{L.~Tomankova,}
\author[aw]{C.~T{\"o}nnis,}
\author[l]{S.~Toscano,}
\author[ai]{D.~Tosi,}
\author[bc]{A.~Trettin,}
\author[x]{M.~Tselengidou,}
\author[f]{C.~F.~Tung,}
\author[y]{A.~Turcati,}
\author[ac]{R.~Turcotte,}
\author[az]{C.~F.~Turley,}
\author[ai]{B.~Ty,}
\author[ba]{E.~Unger,}
\author[al]{M.~A.~Unland~Elorrieta,}
\author[bc]{M.~Usner,}
\author[ai]{J.~Vandenbroucke,}
\author[aa]{W.~Van~Driessche,}
\author[ai]{D.~van~Eijk,}
\author[m]{N.~van~Eijndhoven,}
\author[aa]{S.~Vanheule,}
\author[bc]{J.~van~Santen,}
\author[aa]{M.~Vraeghe,}
\author[at]{C.~Walck,}
\author[b]{A.~Wallace,}
\author[a]{M.~Wallraff,}
\author[ai]{N.~Wandkowsky,}
\author[d]{T.~B.~Watson,}
\author[w]{C.~Weaver,}
\author[ac]{A.~Weindl,}
\author[az]{M.~J.~Weiss,}
\author[aj]{J.~Weldert,}
\author[ai]{C.~Wendt,}
\author[ai]{J.~Werthebach,}
\author[b]{B.~J.~Whelan,}
\author[af]{N.~Whitehorn,}
\author[aj]{K.~Wiebe,}
\author[a]{C.~H.~Wiebusch,}
\author[ai]{L.~Wille,}
\author[ax]{D.~R.~Williams,}
\author[ap]{L.~Wills,}
\author[y]{M.~Wolf,}
\author[ai]{J.~Wood,}
\author[w]{T.~R.~Wood,}
\author[h]{K.~Woschnagg,}
\author[x]{G.~Wrede,}
\author[ai]{D.~L.~Xu,}
\author[g]{X.~W.~Xu,}
\author[au]{Y.~Xu,}
\author[w]{J.~P.~Yanez,}
\author[ab]{G.~Yodh,}
\author[o]{S.~Yoshida,}
\author[ai]{T.~Yuan}
\author[a]{and M.~Z{\"o}cklein}
\affiliation[a]{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\affiliation[b]{Department of Physics, University of Adelaide, Adelaide, 5005, Australia}
\affiliation[c]{Dept. of Physics and Astronomy, University of Alaska Anchorage, 3211 Providence Dr., Anchorage, AK 99508, USA}
\affiliation[d]{Dept. of Physics, University of Texas at Arlington, 502 Yates St., Science Hall Rm 108, Box 19059, Arlington, TX 76019, USA}
\affiliation[e]{CTSPS, Clark-Atlanta University, Atlanta, GA 30314, USA}
\affiliation[f]{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\affiliation[g]{Dept. of Physics, Southern University, Baton Rouge, LA 70813, USA}
\affiliation[h]{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation[i]{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\affiliation[j]{Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany}
\affiliation[k]{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\affiliation[l]{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\affiliation[m]{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\affiliation[n]{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation[o]{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\affiliation[p]{Dept. of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand}
\affiliation[q]{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\affiliation[r]{Dept. of Astronomy, Ohio State University, Columbus, OH 43210, USA}
\affiliation[s]{Dept. of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA}
\affiliation[t]{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}
\affiliation[u]{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\affiliation[v]{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\affiliation[w]{Dept. of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1}
\affiliation[x]{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\affiliation[y]{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\affiliation[z]{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}
\affiliation[aa]{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}
\affiliation[ab]{Dept. of Physics and Astronomy, University of California, Irvine, CA 92697, USA}
\affiliation[ac]{Karlsruhe Institute of Technology, Institut f{\"u}r Kernphysik, D-76021 Karlsruhe, Germany}
\affiliation[ad]{Dept. of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA}
\affiliation[ae]{SNOLAB, 1039 Regional Road 24, Creighton Mine 9, Lively, ON, Canada P3Y 1N2}
\affiliation[af]{Department of Physics and Astronomy, UCLA, Los Angeles, CA 90095, USA}
\affiliation[ag]{Department of Physics, Mercer University, Macon, GA 31207-0001, USA}
\affiliation[ah]{Dept. of Astronomy, University of Wisconsin, Madison, WI 53706, USA}
\affiliation[ai]{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin, Madison, WI 53706, USA}
\affiliation[aj]{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\affiliation[ak]{Department of Physics, Marquette University, Milwaukee, WI, 53201, USA}
\affiliation[al]{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}
\affiliation[am]{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\affiliation[an]{Dept. of Physics, Yale University, New Haven, CT 06520, USA}
\affiliation[ao]{Dept. of Physics, University of Oxford, Parks Road, Oxford OX1 3PU, UK}
\affiliation[ap]{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\affiliation[aq]{Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\affiliation[ar]{Dept. of Physics, University of Wisconsin, River Falls, WI 54022, USA}
\affiliation[as]{Dept. of Physics and Astronomy, University of Rochester, Rochester, NY 14627, USA}
\affiliation[at]{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\affiliation[au]{Dept. of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA}
\affiliation[av]{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\affiliation[aw]{Institute of Basic Science, Sungkyunkwan University, Suwon 16419, Korea}
\affiliation[ax]{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\affiliation[ay]{Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}
\affiliation[az]{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\affiliation[ba]{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\affiliation[bb]{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\affiliation[bc]{DESY, D-15738 Zeuthen, Germany}
\affiliation[bd]{also at Universit{\`a} di Padova, I-35131 Padova, Italy}
\affiliation[be]{also at National Research Nuclear University, Moscow Engineering Physics Institute (MEPhI), Moscow 115409, Russia}
\affiliation[bf]{Earthquake Research Institute, University of Tokyo, Bunkyo, Tokyo 113-0032, Japan}
